The horofunction boundary of the lamplighter group $L_2$ with the Diestel-Leader metric

We fully describe the horofunction boundary $\partial_h L_2$ with the word metric associated with the generating set $\{t,at\}$ (i.e the metric arising in the Diestel-Leader graph $\text{DL}(2,2)$). The visual boundary $\partial_\infty L_2$ with this metric is a subset of $\partial_h L_2$. Although $\partial_\infty L_2$ does not embed continuously in $\partial_h L_2$, it naturally splits into two subspaces, each of which is a punctured Cantor set and does embed continuously. The height function on $\text{DL}(2,2)$ provides a natural stratification of $\partial_h L_2$, in which countably-many non-Busemann points interpolate between the two halves of $\partial_\infty L_2$. Furthermore, the height function and its negation are themselves non-Busemann horofunctions in $\partial_h L_2$ and are global fixed points of the action of $L_2$.

==> defs.tex <==
\usepackage{textcomp}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{stmaryrd}

%%% oft-used sets
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\rationals}{\mathbb{Q}}
\newcommand{\integers}{\mathbb{Z}}

\newtheorem*{corollary*}{Corollary}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{axiom}{Axiom}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}[theorem]{Observation}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}%[section]%compilation error?
\newtheorem{example}{Example}[section]
\newtheorem*{example*}{Example}
\newtheorem*{convention*}{Convention}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}



